Coin-flipping, ball-dropping, and grass-hopping for generating random graphs from matrices of edge probabilities

Common models for random graphs, such as Erd\H{o}s-R\'{e}nyi and Kronecker graphs, correspond to generating random adjacency matrices where each entry is non-zero based on a large matrix of probabilities. Generating an instance of a random graph based on these models is easy, although inefficient, by flipping biased coins (i.e. sampling binomial random variables) for each possible edge. This process is inefficient because most large graph models correspond to sparse graphs where the vast majority of coin flips will result in no edges. We describe some not-entirely-well-known, but not-entirely-unknown, techniques that will enable us to sample a graph by finding only the coin flips that will produce edges. Our analogies for these procedures are ball-dropping, which is easier to implement, but may need extra work due to duplicate edges, and grass-hopping, which results in no duplicated work or extra edges. Grass-hopping does this using geometric random variables. In order to use this idea on complex probability matrices such as those in Kronecker graphs, we decompose the problem into three steps, each of which are independently useful computational primitives: (i) enumerating non-decreasing sequences, (ii) unranking multiset permutations, and (iii) decoding and encoding z-curve and Morton codes and permutations. The third step is the result of a new connection between repeated Kronecker product operations and Morton codes. Throughout, we draw connections to ideas underlying applied math and computer science including coupon collector problems.

==> 99-cut-text.tex <==
The $\chi^2$ random variable and the $\chi^2$ statistical test. A random variable with a $\chi^2$ distribution $k-1$ degrees of freedom if it models a population distributed into $k$ categories at random. dOne of the
most famous instances are the $\chi^2$-variables used in the $\chi^2$-test. \dgnote{Write in example with
	$\chi^2$.}
\arnote{In this type of significance test, a set of observed counts of data distributed over $n$ categories is tested against a set of expected counts over the $n$ categories. The test statistic, $\chi^2 \ = \ \sum \frac{(O-E)^2}{E}$. The null hypothesis is rejected when the test statistic is highly improbable (usually $p>.05$) compared to the $\chi^2$ distribution with $n-1$ degrees of freedom.} 

\arnote{
In a t-test, the means of two samples of data are tested to see if they are significantly different. The true population means of both samples are unknown, so the variance of the samples is used as an estimate of the true variance. If the t-statistic is sufficiently large and has low enough probability of occurring ($p<.05$), then the null hypothesis is rejected and the evidence suggests that the means are significantly different.}



Consider, for instance, the study by \citet{milo} on the presence of \emph{motifs} in networks. \dgnote{Explain Milo Study}
\arnote{This study defines network motifs as patterns of connectivity that are found more frequently in a network than what would be expected in a random network. Milo found motifs in networks from areas ranging from biochemistry, neurobiology, ecology, and engineering. He developed an algorithm to identify motifs and found that each domain contained specific motfis that were over expressed and contributed to unique functions within each domain.}
where the data is sometimes so noisy that many of the interactions do look almost random. One of the easiest and most common methods to do these studies leverages the computer to generate hundreds or hundreds of thousands of instances of a random graph and compute their properties. It almost goes without saying that we need this random graph generation, which is also called random graph sampling, to be as fast and efficient as possible.


%This turns statistical hypothesis testing into a computational challenging
%involving empirical estimates of the probabilities from \emph{many} samples. 

%Social networks, protein-protein interaction networks, the internet, and other large networks have similar properties to a family of synthetic graphs called Kronecker graphs.~\cite{leskovec2005} Kronecker graphs have been proven to follow many of the same properties as real world networks from shrinking diameters to power law degree distributions. \cite{leskovec2010} In addition, Kronecker graphs can be used as a basis of comparison to real world graphs to find domain-specific network motifs, which are patterns of connectivity that appear more in real graphs than in random graphs. \cite{alon} \cite{milo} For example, network motifs could be used to determine
%if your network of friends on Facebook looks similar to one that was
%created at random with the same number of friendships, or if there is some true structure to your friendships.


In order to generate a random adjacency matrix (which represents a graph), we use a graph model which defines the probability that an entry in the adjacency matrix is equal to 1. Here we will describe 4 models. We will focus on the \ERfull model and the Kronecker graph model when we describe later procedures.

Generating random graphs is more complex than random number generation. Figure \ref{fig:intro} shows the connection between well known distributions and probabilities in edge sampling. To generate a random graph we use a model which defines the probability of an edge between nodes. In the next sections we properly define a graph and adjacency matrix, and describe popular graph models.



\begin{listing}
\caption{A simple code to generate a random graph by ball dropping}
\label{code:ball-drop}
\begin{minted}{python}
import numpy as np # numpy is the Python matrix package
"""
Generate a random Erdos-Renyi graph by ball-dropping. The input is:
   n: the number of nodes
   p: the probability of an edge
The result is a list of directed edges. 

Example:
  ball_drop_er(8,0.25) # 8 node Erdos-Renyi with probability 0.25
"""
def ball_drop_er(n,p):
    a = set() # store the set of edges
    matrix = [[0 for x in range(n)] for y in range(n)] 
    edges = math.pow(n,2);
    #m is the number of edges to be generated
    m = int(numpy.random.binomial(edges,p));
    draws=0;
    while(len(a)<m):
        #m edges are randomly selected to be generated
        val = int(random.random()*edges);
        if val not in a:
            a.add(val)
            row = int(val/n);
            col = val % n;
            matrix[row][col]=1;
    return matrix

\end{minted}
\end{listing}


\subsection{coin-flipping} Recall that in an \ERfull graph, any 2 nodes have probability $p$ of being connected. As explained, the simplest way to generate these edges involves flipping $n^2$ weighted coins or ``coin-flipping." Coin-flipping is expensive because it requires ranking of the entire matrix and a coin flip for every pair of nodes leading to a time complexity of $O(log(n)*N^2))$ Because large graphs are very sparse, most coin flips do not result in an edge leading to many unnecessary calculations. We will explain how to solve this inefficiency in section 3.4 on grass-hopping.

\subsection{ball-dropping} In the ball-dropping method, we first sample from a binomial distribution $B(s,p)$ to determine how many edges to create. Then, to determine where to place the edges, we randomly generate permutations of the original probability string. This method is called ball-dropping and is not exact because multiple edges can be placed at the same location. The method can be modified to correct this problem by simply generating another permutation if a duplicate arises. Doing this causes efficiency to be compromised though, especially for small subregions. This problem is actually a restatement of a variation of the classic coupon collector problem, which we discuss in the following section.


\subsection{Coupon Collector's Problem}
%http://math.stackexchange.com/questions/247569/expected-number-of-trials-to-see-x-unique-values-out-of-n-total-values
In our variation of the coupon collector's problem, we must find the expected number of draws needed to obtain $m$ unique objects out of a set of $n$ objects with replacement. Let $X$ be the random variable representing the number of draws needed to obtain the $m^{th}$ unique object. Let $X_i$ be a random variable representing the number of trials needed to obtain the $i^{th}$ unique object given that $i-1$ unique objects have already been drawn. Then, $E(X) = E(X_1) + E(X_2)+...+E(X_m).$ Each random variable $X_i$ is geometrically distributed with $p = 1-\frac{i-1}{n}$ because the probability of drawing a new object is simply the complement of drawing an object that has already been drawn. The expected value of a geometric random variable is $1/p$ so $E(X_i)=\frac{n}{n-i+1}$. Thus, $E(X)=\sum\limits_{i=1}^{m} \frac{n}{n-i+1}$. This can be rewritten in terms of harmonic sums as $n(H_n - H_{n-m})$. Furthermore, $m=pn$ where $p$ is the average probability of the subregion. The harmonic partial sums can be a approximated by the following:  $\sum\limits_{i=1}^{n} \frac{1}{i} \approx \ln n + \gamma$ \cite{pollack}. %Here, the Euler-Mascheroni constant, $\gamma \approx 0.57721$. %use footnote for this?


After substituting in this approximation, the expected number of draws, $E(X)$, simplifies to $n\ln{\frac{1}{1-p}}$. This expression behaves accurately when $p$ is small and close to 0. This can be observed because as $p$ approaches 0, the expression goes to 0, which is intuitively correct because there will be 0 edges to generate. Still, for positive values of $p, E(X) > m$, so the ball dropping method is not as efficient as the direct edge-to-edge hopping, or``grass-hopping", which will be detailed in the following sections.

The underlying distribution is a series of independent Bernoulli trials, thus the need for an exact and efficient sampling method arises.


\subsection{grass-hopping}
Our method, ``grass-hopping'' involves drawing geometric random variables to go directly to the next success or ``head,''  rather than flipping a series of coins one by one. The geometric random variable models the number of trials needed to obtain the next success in a series of coin flips with fixed probability. This procedure is more efficient because large graphs are typically sparse, so most coin flips will not produce edges. Using a geometric random variable allows us to have a time complexity of O(E) where E is the number of edges as opposed to a time complexity of O($n^2$) with coin-flipping. Our method is both efficient and exact because the geometric distribution $\mu =\frac{1}{p}, \sigma=\sqrt{\frac{1-p}{p^2}}$ can be derived from a series of consecutive independent Bernoulli trials. 

A simple intuitive proof for this result is as follows. Consider an \ERfull graph, G(n,p). Recall that a geometric random variable G has distribution $P(G=x)=q^{x-1}p.$ In the adjacency matrix of the graph, the probability that the $i^{th}$ cell will have an edge can be calculated by adding the probabilities of all sequences of hops that land on the $i^{th}$ cell. This sequence of hops is simply a series of geometric random variables whose sum is equal to $i$. All these hop paths can be generated by the expansion of $(p+q)^{i-1}p$ because by the binomial theorem, $(p+q)^{i-1}$ generates all length $i-1$ sequences of p's and q's. Multiplying by p at the end ensures that the final hop lands on the $i^{th}$ cell. $p+q=1$ so the expression $(p+q)^{i-1}p = p$ as expected.

\arnote{make this example for a regular erdos-renyi}
Next, we consider an example case to explain how grass-hopping on an \ERfull graph works. Let our probability matrix be \[P=
\begin{pmatrix}
	p&p&p\\
    p&p&p\\
    p&p&p\\
\end{pmatrix}
\]
There are 3 nodes with 3*2=6 potential directed edges. Instead of flipping a weighted coin at each cell we hop from edge to edge with length equal to the sampled geometric random variable. Let $p=\frac{1}{3},$ Then our geometric random variable will have $\mu =3, \sigma=\sqrt6.$ If our first three draws from this distribution are 2,4 and 3, then edges will be created as as seen in Figure \ref{grass hopping diagram}.

In this way we are guaranteed to have a faster run-time than simply flipping weighted coins at every pair of edges because $E<<N^2$ where E is the number of edges and N is the number of nodes in a graph. 



\newpage
\section{Original Python Code}
In this section is the main sample\_kronecker\_fast method which employs the methods discussed in the earlier sections. In addition, this section contains the kron method which is employed in the get\_geo\_edges method of section 3.1.

\begin{listing}
\caption{Code to generate a random graph by grass-hopping in each \ERfull subregion}
\label{code:sample_kronecker_fast}
\begin{minted}{python}

# sample_kronecker_fast takes as input
#     P : an n-by-n initiator matrix stored as a list-of-lists
#            P[i][j] is the i, jth element. 
#     k : the Kronecker power     
# and returns a set of edges that correspond with a realization
# of a Kronecker graph
def sample_kronecker_fast(P,k):
    array=[]
    g=nx.Graph();
    # creates the first Erdos-Renyi subregion,
    # an array with k 0's 
    for i in range(k):
        array.append(0)
    while(array[0]!=-1):
        # Generate edges in each Erdos-Renyi subregion
        # and then determine the nodes, or row and column indices,
        # of each edge
        for thing in get_geo_edges(P,array):
            row = backward_map(P,thing,'row');
            col = backward_map(P,thing,'col');
            if row > col:
                g.add_edge(row, col);
        # find the next Erdos-Renyi subregion
        array = update(len(P),array);
    return g;

# kron takes as input:
#    p: an n x n iniator matrix of probability values stored
#    as a list of lists.
#    m: an array with k elements representing a probability sequence in # 	 in which each number corresponds to a probability value.
def kron(p,m):
    n = len(p);
    final = 1;
    for i, val in enumerate(m):
        row = int(val/n);
        col = val % n
        final = final * p[row][col]
    return final;

# get_geo_edges takes as input
#    P: an n x n inititator matrix of probability values represented as a
#       list of lists
#    array: the subregion to be sampled represented by an array
#        in which the numbers correspond to letters of the subregion
# and returns a list of edges represented by multisets of numbers
# corresponding to letters.
def get_geo_edges(P,array):
    n=count_permutations(array);
    collection = []
    # p is the common probability value of the subregion
    p=kron(P,array)
    i=-1
    # a is the geometric random variable or length of the hop
    a=numpy.random.geometric(p)
    while(i<=n-a-1):
        i=i+a
        # finds ith multiset permutation
        thearray=unrank(array,i)
        collection.append(thearray);
        # gets the next geometric random variable or hop length
        a=numpy.random.geometric(p);
    return collection

\end{minted}
\end{listing}

\begin{figure}
\caption{Location of \ERfull Subregions in a Kronecker Graph. This figure shows all the common probability or \ERfull subregions for a 3rd power Kronecker graph with a 2x2 initator matrix. In addition, the large subregion shown at the bottom is an example of one subregion from a larger 5th power Kronecker graph. }
\label{ERregions}
\centering
\includegraphics[width=1.4\textwidth]{untitled.pdf}
\end{figure}


\arnote{this paragraph may have some repeats with earlier explanations}
Our method, ``grass-hopping'' involves drawing geometric random variables to go directly to the next success or ``head,''  rather than flipping a series of coins one by one. The geometric random variable models the number of trials needed to obtain the next success in a series of coin flips with fixed probability. This procedure is more efficient because large graphs are typically sparse, so most coin flips will not produce edges. Using a geometric random variable allows us to have a time complexity of O(E) where E is the number of edges as opposed to a time complexity of O($n^2$) with coin-flipping. Our method is both efficient and exact because the geometric distribution $\mu =\frac{1}{p}, \sigma=\sqrt{\frac{1-p}{p^2}}$ can be derived from a series of consecutive independent Bernoulli trials. 

\arnote{This example case may not be necessary because everything has already been explained}
Next, we consider an example case to explain how grass-hopping on an \ERfull graph works. Let our probability matrix be \[P=
\begin{pmatrix}
	p&p&p\\
    p&p&p\\
    p&p&p\\
\end{pmatrix}
\]
There are 3 nodes with 3*2=6 potential directed edges. Instead of flipping a weighted coin at each cell we hop from edge to edge with length equal to the sampled geometric random variable. Let $p=\frac{1}{3},$ Then our geometric random variable will have $\mu =3, \sigma=\sqrt6.$ If our first five draws from this distribution are 3, 3, 4, 2, and 3, then edges will be created as as seen in Figure \ref{fig:grass-hopping}.

In this way we are guaranteed to have a faster run-time than simply flipping weighted coins at every pair of edges because $E<<N^2$ where E is the number of edges and N is the number of nodes in a graph. 





\nenote{I'm adding some references here..not sure it's the best place for them!} The idea of using a geometric distribution that will be described in section \ref{sec:grass-hopping} has been known, but not widely implemented.~\citet{BatageljBrandes2005} suggested the models’ applicability to small world graphs and preferential attachment graphs.  They also pointed out that many popular software routines could be greatly improved, as they were using a coin-flipping scheme. The algorithm  was extended by ~\citet{MillerHagberg2011} to Chung-Lu graphs that runs in $\bigO(N+M)$ time. Yet another graph model called the Random Kernel Graph was introduced by~\citet{HagbergLemons2015}, which is a generalization of the models of ER and Chung-Lu. They discuss a variation of grass-hopping and additionally efficient generation when considering symmetric graphs. In the next several sections we aim to highlight alternative more efficient graph generation to coin-flipping.


In the case that the value is the maximum, the value is changed to $-1$ to indicate that all \ERfull subregions have been completed. If the length of the array is greater than $1$, then the last element is incremented. In the case that the last element is the maximum, then the last element is changed to the final element of the updated version of a sub-array with the last element of the initial array removed. This step is taken to ensure that the returned sequence is non-decreasing so that no \ERfull subregion is generated twice. 





The first two digits have place values of $n^{2k+1}$ and $n^{2k}$ respectively showing that they occupy the beginning positions of the new digit-strings.

Mathematically,
\begin{equation}
M(I_{k+1})=(\lfloor {\frac{r_{k+1}}{n}} \rfloor n^{2k+1}+i, (r_{k+1} \% n)+j)
\label{eqn:final}
\end{equation}


==> 99-fast-kron-arjun.tex <==
% A bunch of great text that Arjun wrote that I'm abusing here...

\begin{compactenum}
\item Enumerate each \ERfull region in the $k$-dimensional multiplication table (or equivalently, the Kronecker graph). 
\item For each region, 
\end{compactenum}
We will now explain how grass-hopping can be applied  to Kronecker Graphs in order to increase the efficiency of sampling. 

Recall that a Kronecker Graph is simply  a union  of many \ERfull subgraphs.

\arnote{do we need these paragraphs?}
This process involves several steps. We explain how to unrank the permutations of an array. In other words, we explain how to find the $k^{th}$ permutation in lexicographic order of an array. For example consider the sequence $[1,1,2,3]$. What is the $3^{rd}$ permutation in lexicographic order of this array? The answer in this case is $[1,2,1,3]$. 

We show how to locate the indices of a probability string permutation in a Kronecker graph by using a backward-mapping algorithm that exploits the recursive nature of the Kronecker product. This backward map uses a z-curve or Morton code in a new connection to Kronecker graphs.

By combining these three solutions, we can sample a Kronecker graph because it is simply a union of many \ERfull subgraphs. 

\subsection{Grass Hopping}

In order to illustrate this procedure, we will work through an example case. If we called  $get\_geo\_edges([[.5,.8],[.3,.7]],[0,1,2])$ Then we are generating edges in the ``$abc$'' subregion of a $3^{rd}$ power Kronecker graph. This is because the numbers in the array [0,1,2] correspond to the letters of the subregion ``$abc$.'' The probability values are assigned as \[P=
\begin{pmatrix}
	a&b\\
    c&d\\
\end{pmatrix} = 
\begin{pmatrix}
	.5&.8\\
    .3&.7\\
\end{pmatrix}
\] so  $abc$ = .12. The number of permutations of ``$abc$'' is 3!=6, so we must flip 6 weighted coins with probability .12. Instead of flipping these weighted coins, though, we employ the more efficient solution of drawing geometric random variables with distribution $P(G=x)=(1-p)^{x-1}*p$ where $p = .12$ by calling $numpy.random\_geometric(.12)$. The value of the geometric random variable tells us the rank or index of the next 'heads' or edge. Once we have this index we must use the unranking algorithm to find which permutation or edge corresponds to that index or rank.

\begin{listing}
\begin{minted}{python}

# get_geo_edges takes as input
#    K: an n x n inititator matrix of probability values represented as a
#       list of lists
#    array: the subregion to be sampled represented by an array
#        in which the numbers correspond to letters of the subregion
# and returns a list of edges represented by multisets of numbers
# corresponding to letters.
def get_geo_edges(K,array):
    n=count_permutations(array);
    collection = []
    # p is the common probability value of the subregion
    p=kron(K,array)
    i=-1
    # a is the geometric random variable or length of the hop
    a=numpy.random.geometric(p)
    while(i<=n-a-1):
        i=i+a
        # finds ith multiset permutation
        thearray=unrank(array,i)
        collection.append(thearray);
        # gets the next geometric random variable or hop length
        a=numpy.random.geometric(p);
    return collection
    
\end{minted}
\end{listing}

\subsection{Unranking the Edges}


After generating edges within each \ERfull subregion, the locations of the edges in the original Kronecker graph must be identified. In other words, we must map the $k^{th}$ permutation in a given subregion back to a cell in the larger Kronecker matrix. The cell's location tells us which two nodes the edge connects. This involves a two step process as seen in Figure \ref{Unranking Diagram}.


\begin{figure}
\caption{Unranking the ``aabb'' subregion. The second permutation of ``aabb'' is ``abab.'' The indices of ``abab'' in the $P^4 KPGM)$ is (0,5)}
\label{Unranking Diagram}
\centering
\includegraphics[width=.35\textwidth]{unrank.png}
\end{figure}

\subsubsection{Lexicographic Map}
The first step is to form a one-to-one correspondence between the edges in a subregion and the multiset permutations of the subregion probability string. This mapping can be created by ordering the permutations lexicographically and unranking the $``n^{th}"$ edge to the $``n^{th}"$ lexicographic permutation of the subregion probability string as seen in the unrank algorithm below.

The unrank algorithm takes as input a multiset permutation in non-decreasing form represented as an array, as well as an index or ``rank" of which to find the corresponding permutation. The algorithm is recursively defined and simply returns the original array if the inputted rank is 0 as the base case. In the recursive case, the algorithm finds the ``next" value for the new ``unranked" permutation and then appends that value to the beginning of the new array. It does this by looping through each element of the array and counting the cumulative number of permutations when each element is left out. When this cumulative total passes the index or rank we are looking for, then the corresponding ``removed" element is the next one in the array.

\begin{listing}
\begin{minted}{python}
# unrank takes as input:
#    C: a multiset represented by a list
#    n: the lexicographic rank or index to be found
# and returns the nth permutation of C in lexicographic order.

# Precondition: C must be in non-decreasing order
# This function is implemented recursively, so it is not
# appropriate for extremely long sequences

# Examples:
# unrank([0,1,1,3], 0) returns [0,1,1,3]
# unrank([0,1,1,3], 1) returns [0,1,3,1]
# unrank([0,1,1,3], 2) returns [0,3,1,1]

def unrank(C, n):
    counter = 0;
    # base case of recursion
    if n == 0:
        return numpy.array(C);
    
    # find the element at the start of the unranked permutation
    for i,s in enumerate(C):
        # we want to test if element s starts the
        # new permutation

        # checks for repeated elements to prevent overcounting
        if(i!=0 and s==C[i-1]):
            continue;
        # creates placeholder list and removes s at position i
        place = numpy.delete(C,i)
        # checks if s starts the new permutation. Then start
        # the recursive step to unrank the rest of the list
        if(count_permutations(place) > n-counter):
            return numpy.append(s, unrank(place, n-counter));
        # updates the counter of the total number of permutations
        counter += count_permutations(place);

\end{minted}
\end{listing}

\subsubsection{Backward Mapping}
After identifying the appropriate permutation corresponding to each edge, the permutations must be mapped back to locations in the adjacency matrix. The motivation for the proposed method comes from the fractal structure of KPGMs. \cite{leskovec2010} For example, consider the $k^{th}$ power of a Kronecker initiator matrix with entries $a,b,c, \text{and } d$. If a given probability string has a first entry of $a$, then the string is located in top left corner of the matrix. Similarly, if the first letter of the string is $b$, the string is located in the top right corner of the matrix and so on for $c$ and $d$. $K^k = \begin{pmatrix}
a\cdot K^{k-1} &b\cdot K^{k-1}\\ c\cdot K^{k-1} &d\cdot K^{k-1}
\end{pmatrix}$

In this way we can recursively define a backwards mapping algorithm to determine the location of any edge probability string in the KPGM as seen in Algorithm \ref{alg:back-map}


\begin{algorithm}
\caption{Backward-Map algorithm}
\label{alg:back-map}
\begin{algorithmic}[1]
\Procedure{Backward-Map}{$s$}\Comment{Finds the indices of a probability string s}
\State $r\gets 0, c\gets 0$
\For{i from 0 to len(s)}
\If{s[i]==c or s[i]==d}
\State $r \gets r + 2^{len(s)-i-1}$
\EndIf
\If{s[i]==a or s[i]==b}
\State $c \gets c + 2^{len(s)-i-1}$
\EndIf
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

This algorithm can be expanded to a general case as follows. Each initiator matrix probability value can be defined by its indices $m_{ij}$. Thus when looping through a probability string, the next region to ``zoom'' into is known based on the initiator matrix row and column indices of the specific probability value. The general equation for the row value is $R=\sum\limits_{i=0}^{k-1} {r_i} \times n^{k-i-1}$ where r is the array of row values in the initiator matrix of the given probability string. The column value equation is essentially the same: $C=\sum\limits_{i=0}^{k-1} {c_i} \times n^{k-i-1}$ where $c$ is the array of column values in the initiator matrix of the given probability string. This general case solution as shown below.

\begin{listing}
\begin{minted}{python}
# backward_map takes as input
#    K: an n x n initiator matrix stored as a list of lists
#    s: an array (probability sequence) consisting of a permutation of letters
#        represented as numbers 0,1,2...(n^2 - 1)
#    flag: a string showing whether to find the row index or column index
# and returns the corresponding row or column index of the probability sequence
# in the kronecker product graph matrix

def backward_map(K,s,flag):
    n = len(K);
    if(flag=='row'):
        x=0;
        # we want to "zoom" further into the matrix for each
        # value of our cell
        for i, val in enumerate(s):
            length = len(s)-i;
            row = int(val/n);
            x += row * math.pow(n,length-1);
        return int(x)
    elif(flag=='col'):
        y=0;
        # we want to "zoom" further into the matrix for each
        # value of our cell
        for i, val in enumerate(s):
            length = len(s)-i;
            col = val % n;
            y += col * math.pow(n,length-1);
        return int(y)
\end{minted}
\end{listing}

\subsubsection{Morton Codes}

\arnote{Use K for Kronecker matrix and v for vectorized version}

In this section we prove a novel connection between Kronecker product graph matrices and Morton codes. A Morton code maps multidimensional data to one-dimensional data. Suppose $K^k$ is a matrix of dimension $n^k \times n^k$ and $v^k$ is a vector of length $(n^2)^k$. $K^k$ and $v^k$ have the same number of entries, and we wish to map between them while preserving a certain amount of locality. The Morton Code (or Z-order) is one such map. As seen in Figure \ref{Morton Code Matrix}, it is called the Z-order because of the shape of the curve. The Morton Code is an example of an interleaving sequence. Moving through the multidimensional space alternates between a larger index in either dimension.

In our case, $K^k$ is the result of $k-1$ Kronecker products of the initiator matrix $K: n \times n$, and $v$ is the result of $k-1$ Kronecker products of the vectorized version of $K_1$. Then the Morton Code is a map 
\begin{eqnarray}
M: \, &v^k& \rightarrow K^k \nonumber \\
&I& \, \mapsto (i,j) \nonumber 
\end{eqnarray}
where $(i,j)$ is an index of a cell in the KPGM, and $I$ is a permutation of initiator matrix probability values. The reverse of the Morton code or the ``decoding'' allows us to determine the index of a given probability sequence give the row and column values.

%In this section we will first explain Morton coding and decoding, and then prove that the method produces the appropriate indices for a given probability sequence. 

The lexicographic order of the permutations in a Kronecker matrix is the same as the order of interleaved base n row and column values. So in order to ``decode'' an index $I$, first $I$ is written in base $n$. Then, alternating digits are separated creating two base n numbers. These two numbers are converted back to the original base completing the process. This process can be seen in figure \ref{Morton Code Matrix}.  For example, if the row and column values of a cell are $i=4=11_2$ and $j=1=01_2$, then after the interleaving the digits of i and j, $I=1011_2=1$. Thus, $M(4,1)=11$.

\begin{theorem} 
Let $I$ be the lexicographic index of a probability sequence representing an edge in a Kronecker matrix of power $k$. The Morton decoding of $I$ provides the appropriate row and column indices of the sequence, i.e. $decode(I_k) \rightarrow (i_k,j_k)$.
\end{theorem}

%$Proof:$ 
\begin{proof}
We will prove this statement by induction on the power of the Kronecker product, k.

$Base \ Case:$ When k = 1, $K^k = K^1 = K$ is simply the initiator matrix. 
\\
\[v=
\begin{pmatrix}
	p_0\\
    p_1\\
    \vdots\\
    p_{n^2-1}
\end{pmatrix} \rightarrow K = \begin{pmatrix}
	p_0&p_1&\ldots&p_{n-1}\\
    p_n&\ldots&\ldots &p_{2n-1}\\
    \vdots&\ddots&\ddots&\vdots\\
    p_{n^2-n}&\ldots&\ldots&p_{n^2-1}
\end{pmatrix}\]
Here the probability values are simply arranged in the matrix in numerical order, so $I$ uniquely decomposes to $(i,j)$ by $I = i*n+j$, where n is the size of the initiator matrix. This satisfies the Morton code because the interleaving of the values $i$ and $j$ produces the value $ij_n$ in base $n$, which also equals $in+j$.

$Inductive \ Step:$ Assume $M$ correctly maps between $K^k$ and $v^k$. Recall that $K^{k+1} = K^{k} \otimes K$. So each probability sequence in $K^{k+1}$, is simply the product of the probability sequences in the previous Kronecker matrix, $K^{k}$, and the initiator matrix probability values.

Let $p_1p_2 \ldots p_k p_{k+1}$ be a sequence in $v^{k+1}$. Then notice that $p_1p_2 \ldots p_k$ is a sequence in $v^k$. By assumption, the Morton code correctly gives the correct row and column values in $K^k$: $i_k$ and $j_k$. Then the row value for $p_1p_2 \ldots p_k p_{k+1}$ is $i_{k+1}$ where
\begin{align} 
i_{k+1} = i_k + \left\lfloor {\frac{val}{n}} \right\rfloor n^k
\label{eqn:rowval}
\end{align}
and $val$ is the index of $p_{k+1}$ in $v^{k+1}$. The reasoning for this is as follows. The size of the previous iteration's matrix, $n^k$, determines how large each ``row" is. When we multiply a probability sequence by a new value, think of ``zooming'' into a specific region of the Kronecker matrix. The region we ``zoom'' into is dependent on the position of the probability value. %The row location of a probability value can be found by simply taking the floor of the probability index divided by n.


The same reasoning can be translated to find the column index, $j_{k+1}$. 
\begin{align}
j_{k+1} = j_k + (val \% n) *n^k
\label{eqn:colval}
\end{align}
where $\%$ represents the modulus operator. By finding $val$ mod $n$, we know how many columns over the added probability value is. The morton code interleaves the digits of $i_{k+1}$ and $j_{k+1}$ in base $n$. $i_{k+1}$ in base $n$ is simply the digits of $i_k$ in base $n$ with the value $\lfloor {\frac{val}{n}} \rfloor$ added to the front. This is because the added value will occupy the $n^k$ digits place because that is what it is multiplied by in \ref{eqn:rowval}. Thus, the interleaved digits of $i_{k+1}$ and $j_{k+1}$ will be $\lfloor {\frac{val}{n}} \rfloor$, $(val \% n)$, followed by the interleaved digits of $i_k$ and $j_k$. Since, $I$ = interleaved digits of $i_k$ and $j_k$ in base $n$, it suffices to show that: 
\begin{align}
I_{k+1} = \lfloor {\frac{val}{n}} \rfloor *n^{2k+1} + (val \% n)*n^{2k} + I
\label{eqn:interleaved}
\end{align}
We multiply the first two digits by $n^{2k+1}$ and $n^{2k}$ respectively because those are the place values they occupy when moving from base $n$ to base $10$. Now we must find a way to express $I_{k+1}$ recursively in terms of $I_k$, $val$, and $n$. 

\begin{figure}
\centering
\includegraphics[width=.8\textwidth]{morton-code-diagram.png}
\caption{The Morton decoding process of a $2^{nd}$ power Kronecker graph. The decoding process takes the lexicographic index of a probability sequence and maps it to 2-dimensional $(i,j)$ indices by a z-order curve. In (a) and (c), the probability sequences are ranked directly in lexicographic order. Writing the index in base $2$ and separating every other digit yields the row and column indices for each permutation as seen in (b). The placing of permutations in the matrix that arises is the same as that of the $2^{nd}$ power Kronecker matrix (d). The ordering of the lexicographic indexes in (b) is a z-shaped fractal pattern (Follow the ordering of the numbers from $0-15$.) }
\label{fig:morton-small}
\end{figure}

A given probability string s has a lexicographic index $I_k$. When we move to the next Kronecker power, we multiply this probability sequence by a third value, $val$. We can determine the new lexicographic index $I_{k+1}$ if we know $I$ and $val$. $I_{k+1} = I_k + val*(n^2)^k$ This result arises because we must add the number of permutations that start with values that precede $val$. The number of permutations that start with values before $val$ is simply the number of values that precede $val$, which span from $0$ to $val-1$, times the number of length $k$ permutations of initiator matrix probability values. There are $n^2$ probability values and $k$ slots to place them in with replacement so there are $v(n^2)^k$ permutations that start with values before $val$. We can now substitute this equation into equation \ref{eqn:interleaved} yielding $I_k + val*(n^2)^k = \lfloor {\frac{val}{n}} \rfloor *n^{2k+1} + (val \% n)*n^{2k} + I_k$. Simplifying yields $val = \lfloor {\frac{val}{n}} \rfloor *n + (val \% n)$. 

From here our proof is trivial because this equation is just a restatement of the remainder theorem. $val$ can be written as the integer portion of $val/n$ plus the remainder of $val$ divided by $n$. This completes our proof because we have shown that Morton code provides the correct map from $(i,j)$ indices of a probability sequence in the KPGM to the lexicographic index $I$ of the sequence.
\end{proof}

\subsection{Finding the Next Subregion}
After unranking the edges in an \ERfull subregion, the next step is to find the subsequent \ERfull subregion. For example, after finishing the ``$aabc$'' subregion of a $4^{th}$ power Kronecker graph, we must move on to the ``$aabd$'' subregion, because it is the next nondecreasing sequence of initiator matrix probability values. Once we have updated to the next subregion, we will repeat the process of hopping edges and unranking. 

This update algorithm works by first checking if the given array has a length of $1$. If so, the value is incremented by $1$. In the case that the value is the maximum, the value is changed to $-1$ to indicate that all \ERfull subregions have been completed. If the length of the array is greater than $1$, then the last element is incremented. In the case that the last element is the maximum, then the last element is changed to the final element of the updated version of a sub-array with the last element of the initial array removed. This step is taken to ensure that the returned sequence is non-decreasing so that no \ERfull subregion is generated twice. 

\subsection{Generating an Example Graph}
In this section, we generate a sample graph to illustrate the overall algorithm. Let's start with the 3 x 3 initiator matrix \\
\[P=
\begin{pmatrix}
	.4&.7&.55\\
    .3&.8&.9\\
    .5&.2&.6
\end{pmatrix}
\]
We would like to generate second power kronecker graph, which will have 9 nodes using this initiator matrix P, so we call $sample\_kronecker\_fast([[.4,.7,.5],[.3,.8,.9],[.5,.2,.6]],2)$. \\
\[P \otimes P = \begin{pmatrix}
	.16&.28&.22&.28&.49&.385&.22&.38&.3025\\
    .12&.32&.36&.21&.56&.63&.165&.44&.495\\
    .2&.08&.24&.35&.14&.42&.275&.11&.33\\
    .12&.21&.165&.32&.56&.44&.36&.63&.495\\
    .09&.24&.27&.24&.64&.72&.27&.72&.81\\
    .15&.1&.18&.4&.16&.48&.45&.18&.54\\
    .2&.35&.275&.08&.14&.11&.24&.42&.33\\
    .15&.4&.45&.06&.16&.18&.18&.48&.54\\
    .25&.1&.3&.1&.04&.12&.3&.12&.36\\
\end{pmatrix}\]

Here, each entry in $P \otimes P$ represents the probability that a cell in the random graph will contain an edge, or 1. As noted in section 1, the edges can be generated by either flipping a weighted coin at every single cell, or by hopping directly from edge to edge in each common probability region by drawing geometric random variables. An example of a randomly generated graph can be seen in figure \ref{example graph}.

\begin{figure}[ht]
\centering
\includegraphics[width=.45\textwidth]{6-12_sample_graph.png}
\caption{Sample Kronecker Graph with 9 nodes created using probability matrix found in section 4}
\label{example graph}
\end{figure}

\subsection{Efficiency Analysis}
Here we calculate the order of complexities of this algorithm and the previous coin flipping method. \newline
Coin Flipping – Recall that this method involves going through every pair of nodes (or cell of the adjacency matrix) and flipping a weighted coin. This algorithm takes $\bigO(k N^2) = \bigO(N^2 \log N)$ time, because finding the probability of a cell takes k, or $\log N$ time. (N is the number of nodes)
\newline
Grass Hopping – Recall that this method has the advantage of hopping directly to the next edge using the geometric random variable. The method takes approximately $\bigO(kE)$ time because we need only backward map the created edges. $E$ is the expected number of edges which can be calculated using indicator functions. For a given cell X, if $p(X=1)=s$, then the expected value of the cell is s. Because the total number of expected edges is just the sum of the indicator random variables of every cell, $E(E) = \sum_{i} p_i = 1$. 

In order to quickly sum up every single probability value, recall from Section 3.1 that every length k permutation with not necessarily distinct elements of a’s, b’s, c’s, and d’s appears in the matrix. By the multinomial theorem, the expansion of $(a+b+c+d)^k$ produces all of these such sequences. To prove that the time complexity is less than that of coin-flipping, multiply this expression by $N^2/N^2$. $N = 2^k$ so $N^2 = 4^k.$ Thus $E(E) = (a+b+c+d)^k \frac{N^2}{4^k} = N^2 (\frac{a+b+c+d}{4})^k$.
The average of a, b, c, and d is less than or equal to one, thus the expected number of edges is significantly less than $N^2$, especially for a large Kronecker power.  Let $\bar{p} = \frac{a+b+c+d}{4}$, then the order of complexity is $\bigO(N^2 \times \bar{p}^{\log n} \times \log n)$ which is significantly less than $\bigO(N^2 \times \log n)$.

\section{Fixed Edge Generation of Erd\H{o}s-R\'{e}nyi Graphs}
In the first section, we noted how the original \ERfull graph was one randomly sampled from the set of graphs with m edges and n nodes. We stumbled upon a potentially unknown method of generating such graphs using techniques detailed earlier in this paper. In a graph with n nodes, there are $\binom{n}{2}$ pairs of nodes or possible edges. Any subset of m pairs of nodes defines a unique graph. Thus there are $\binom{\binom{n}{2}}{m}$ possible graphs. How do randomly generate one of these graphs? Our solution is to ``rank" each graph by assigning it a numerical value from 0 to $\binom{\binom{n}{2}}{m}-1$. Once we randomly generate one of these ranks, we must unrank this value back to the m edges, and then unrank these edges back to pairs of nodes. Each graph is defined by set of edges, each of which can also be assigned a rank from 0 to $\binom{n}{2}-1$. We need a one-to-one correspondence between the graph rank and the set of edges that defines the graph. We can simply use a lexicographic map of non-decreasing sequences, similar to the solution to the unranking problem in section 3.2.1 i.e. if m=3, the following  ranks of graphs map to the following edges. $0->(0,1,2), 1->(0,1,3)$ and so on. We can generalize this mapping by writing an algorithm that takes 3 inputs: a rank, the maximum number of an edge, and the number of edges of our graph. The $unrank$ algorithm shown below will find the non-decreasing sequence in lexicographic order which satisfies the given parameters. Like the previous unranking algorithm, we must find the next element of our set by counting the number of possible sequences starting with that value. Instead of using the multinomial theorem though, we must use a combination because since the order of edges does not matter, each edge sequence has a unique non-decreasing ordering. 

The $erdos\_renyi$ algorithm uses the $unrank$ algorithm to generate a random graph from the set of $\binom{\binom{n}{2}}{m}-1$ graphs with n nodes and m edges. After randomly generating the "rank" of the graph, and finding the set of edges using the $unrank$ method, we must find the nodes that correspond to these edges. We can simply use the same $unrank$ algorithm to establish a one-to-one correspondence between the edge ranks and the ranks of the nodes. In this case, length = 2, because each edge has 2 nodes, and $max\_val$ = n because there are n nodes.

\begin{listing}
\caption{A simple code to generate an \ERfull graph with a fixed number of edges}
\label{code:fixed_er}
\begin{minted}{python}

# combination takes as input
#   n: the total number of objects to choose from
#   k:the number of objects to choose
# and returns the combination n choose k.
def combination(n,k): 
  return int( reduce(mul, (Fraction(n-i, i+1) for i in range(k)), 1) )

# unrank takes as input
#   I: the rank of the graph
#   max_val: the number of potential edges
#   length: the number of edges
# and returns the Ith non-decreasing sequence of edges
# of length 'length' and maximum edge of value of (max_val-1)
def unrank(I, max_val, length):
  array = [];
  # finds the next edge value
  for i in range(max_val):
    if length == 0:
      break;
    if length == 1:
      array.append(i + I);
      length=length-1;
    # checks if next edge value is i
    elif(combination(max_val-i-1, length-1) > I):
      array.append(i);
      length = length - 1; 
    else:
      I = I - combination(max_val-i-1, length-1);
  return array;

# erdos_renyi takes as input:
#   n: the number of nodes
#   m: the number of edges
# And generates a graph at random from the set of graphs
# with n nodes and m edges.

def erdos_renyi(n,m):
  graph = nx.Graph();
  #computes the number of possible edges
  possible_edges = int(n*(n-1)/2);
  #computes the number of possible graphs
  possible_graphs = int(combination(possible_edges,m));

  #randomly generates a "rank" or number of the graph
  I = int(random.random()*possible_graphs)

  #finds the m edges that make up the graph
  edges = unrank(I, possible_edges, m);

  #finds the nodes of edges: a set of edges.
  for edge in edges:
    nodes = unrank(edge, n, 2);
    print(nodes);
    graph.add_edge(nodes[0],nodes[1]);
  return graph;
\end{minted}  
\end{listing}




























% The following text was removed on March 6th. 



%First, we convert both numbers into base 2 digit-strings: $4\rightarrow 0100_2$; $11 \rightarrow 1011_2$. Next, we interleave the digits of the two numbers to obtain our final digit-string. $Interleave(0100_2,1011_2)\rightarrow 01100101_2$. Converting this number to base 10 yields our final encoded value: 101. Note that we do not have to operate in base 2; we could perform the same base changing and interleaving in any other base. The Morton Code is sometimes called the z-order code because tracing the pattern of encoded values in numerical order in a table forms a z-like pattern. Fig. \ref{fig:morton-small}

The Morton Code is an example of an interleaving sequence that encodes multidimensional data in a single linear index. Moving through the multidimensional space alternates between a larger index in either dimension. Suppose $K^k$ is a matrix of dimension $n^k \times n^k$ and $v^k$ is a vector of length $(n^2)^k$. $K^k$ and $v^k$ have the same number of entries, and we wish to map between them while preserving a certain amount of locality. The Morton Code (or Z-order) is one such map. 

\dgnote{Outline: 1-2 paragraphs explaining how we use Equation 5.7}
\dgnote{Outline: 1-2 paragaphs explaining the code to translate a unranked multiset perm to row/col}
\dgnote{Outline:  This code should generate Big I first, then compute I' after the Morton code permutation, and 
  then }

In this section we prove a novel connection between repeated Kronecker product graph matrices and Morton codes. A Morton code maps multidimensional data to one-dimensional data. As seen in Figure \ref{fig:morton-small}, it is also called the Z-order because of the shape of the curve. 


\begin{listing}
\begin{minted}[fontsize=\footnotesize]{python}
function multindex_to_linear(ind,n2):
  I = 0
  base = 1
  for i = xrange(length(ind),-1,0):
    I += i*base
    base *= n2
  return I
function morton_permute(I,n):
  num=[]
    while I>= n:
        num.insert(0,I%n);
        I=int(I/n);
    num.insert(0,I);
    return num;
def morton(I,n,k):
  Ip = 0
  ind = 0
  base0 = 1
  base1 = n**k
  while I >= n:
    digit = I%n
    I = I // n # integer division
    if ind%2 == 0:
      Ip += base0*digit
      base0 *= n
    else:
      Ip += base1*digit
      base1 *= n
    ind += 1
  return Ip    
function kronlinear_to_rowcol(Ip,n,k)
  nk = n**k # compute n^k
  row = Ip \% nk
  col = ip // nk 
  return (row,col)
\end{minted}
\end{listing}




The Morton Code is an example of an interleaving sequence that encodes multidimensional data in a single linear index. Moving through the multidimensional space alternates between a larger index in either dimension. Suppose $K^k$ is a matrix of dimension $n^k \times n^k$ and $v^k$ is a vector of length $(n^2)^k$. $K^k$ and $v^k$ have the same number of entries, and we wish to map between them while preserving a certain amount of locality. The Morton Code (or Z-order) is one such map. For example, let's say we want to encode the numbers 4 and 11 into a single value. First, we convert both numbers into base 2 digit-strings: $4\rightarrow 0100_2$; $11 \rightarrow 1011_2$. Next, we interleave the digits of the two numbers to obtain our final digit-string. $Interleave(0100_2,1011_2)\rightarrow 01100101_2$. Converting this number to base 10 yields our final encoded value: 101. Note that we do not have to operate in base 2; we could perform the same base changing and interleaving in any other base. The Morton Code is sometimes called the z-order code because tracing the pattern of encoded values in numerical order in a table forms a z-like pattern. Fig. \ref{fig:morton-small}


In our case, $K^k$ is the result of $k-1$ Kronecker products of the initiator matrix $K: n \times n$, and $v$ is the result of $k-1$ Kronecker products of the vectorized version of $K_1$. Then the Morton Code is a map 
\begin{eqnarray}
M: \, &v^k& \rightarrow K^k \nonumber \\
&I& \, \mapsto (i,j) \nonumber 
\end{eqnarray}
where $(i,j)$ is an index of a cell in the KPGM, and $I$ is a permutation of initiator matrix probability values. The reverse of the Morton code or the ``decoding'' allows us to determine the index of a given probability sequence give the row and column values.

Equation \ref{eq:morton-kron} shows the mapping illustrated in figure \ref{fig:morton-small}. The repeated Kronecker product of a series of vectorized Kronecker matrices produces a vector  with elements in lexicographic order. The permutation matrix $\mM$ maps the vectorized Kronecker matrix to this vector with elements in lexicographic operation. The opposite operation, the $morton\_decode$ function, maps the lexicographic vector to the actual Kronecker matrix. 

The lexicographic order of the permutations in a Kronecker matrix is the same as the order of interleaved base n row and column values. So in order to ``decode'' an index $I$, first $I$ is written in base $n$. Then, alternating digits are separated creating two base n numbers. These two numbers are converted back to the original base completing the process. This process can be seen in figure \ref{fig:morton-small}.  For example, if the row and column values of a cell are $i=4=11_2$ and $j=1=01_2$, then after the interleaving the digits of i and j, $I=0111_2=7$. Thus, $M(4,1)=7$. Note that the digits are interleaved with the first column value at the start. This is because we are vectorizing are Kronecker matrix column-wise.

The Morton Decode algorithm is shown in listing 6. First, the multiset index is converting into a single linear index. This conversion is just a base $n^2$ to base 10 conversion. Next, the linear index  is converted into base n number. After that, the opposite of the interleaving process is performed; every other digit is taken to form the row and column indices













==> 99-fast-kron-left.tex <==
% In this file, I'm deleting text from Arjun as I use it.
\subsection{Grass Hopping}

\subsubsection{Backward Mapping}
After identifying the appropriate permutation corresponding to each edge, the permutations must be mapped back to locations in the adjacency matrix. The motivation for the proposed method comes from the fractal structure of KPGMs. \cite{leskovec2010} For example, consider the $k^{th}$ power of a Kronecker initiator matrix with entries $a,b,c, \text{and } d$. If a given probability string has a first entry of $a$, then the string is located in top left corner of the matrix. Similarly, if the first letter of the string is $b$, the string is located in the top right corner of the matrix and so on for $c$ and $d$. $K^k = \begin{pmatrix}
a\cdot K^{k-1} &b\cdot K^{k-1}\\ c\cdot K^{k-1} &d\cdot K^{k-1}
\end{pmatrix}$

In this way we can recursively define a backwards mapping algorithm to determine the location of any edge probability string in the KPGM as seen in Algorithm \ref{alg:back-map}


\begin{algorithm}
\caption{Backward-Map algorithm}
\label{alg:back-map}
\begin{algorithmic}[1]
\Procedure{Backward-Map}{$s$}\Comment{Finds the indices of a probability string s}
\State $r\gets 0, c\gets 0$
\For{i from 0 to len(s)}
\If{s[i]==c or s[i]==d}
\State $r \gets r + 2^{len(s)-i-1}$
\EndIf
\If{s[i]==a or s[i]==b}
\State $c \gets c + 2^{len(s)-i-1}$
\EndIf
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

This algorithm can be expanded to a general case as follows. Each initiator matrix probability value can be defined by its indices $m_{ij}$. Thus when looping through a probability string, the next region to ``zoom'' into is known based on the initiator matrix row and column indices of the specific probability value. The general equation for the row value is $R=\sum\limits_{i=0}^{k-1} {r_i} \times n^{k-i-1}$ where r is the array of row values in the initiator matrix of the given probability string. The column value equation is essentially the same: $C=\sum\limits_{i=0}^{k-1} {c_i} \times n^{k-i-1}$ where $c$ is the array of column values in the initiator matrix of the given probability string. This general case solution as shown below.

\begin{listing}
\begin{minted}{python}
# backward_map takes as input
#    K: an n x n initiator matrix stored as a list of lists
#    s: an array (probability sequence) consisting of a permutation of letters
#        represented as numbers 0,1,2...(n^2 - 1)
#    flag: a string showing whether to find the row index or column index
# and returns the corresponding row or column index of the probability sequence
# in the kronecker product graph matrix

def backward_map(K,s,flag):
    n = len(K);
    if(flag=='row'):
        x=0;
        # we want to "zoom" further into the matrix for each
        # value of our cell
        for i, val in enumerate(s):
            length = len(s)-i;
            row = int(val/n);
            x += row * math.pow(n,length-1);
        return int(x)
    elif(flag=='col'):
        y=0;
        # we want to "zoom" further into the matrix for each
        # value of our cell
        for i, val in enumerate(s):
            length = len(s)-i;
            col = val % n;
            y += col * math.pow(n,length-1);
        return int(y)
\end{minted}
\end{listing}

\subsubsection{Morton Codes}

\arnote{Use K for Kronecker matrix and v for vectorized version}




%In this section we will first explain Morton coding and decoding, and then prove that the method produces the appropriate indices for a given probability sequence. 

The lexicographic order of the permutations in a Kronecker matrix is the same as the order of interleaved base n row and column values. So in order to ``decode'' an index $I$, first $I$ is written in base $n$. Then, alternating digits are separated creating two base n numbers. These two numbers are converted back to the original base completing the process. This process can be seen in figure \ref{Morton Code Matrix}.  For example, if the row and column values of a cell are $i=4=11_2$ and $j=1=01_2$, then after the interleaving the digits of i and j, $I=1011_2=11$. Thus, $M(4,1)=11$.
 

\begin{theorem} 
Let $I$ be the lexicographic index of a probability sequence representing an edge in a Kronecker matrix of power $k$. The Morton decoding of $I$ provides the appropriate row and column indices of the sequence, i.e. $decode(I_k) \rightarrow (i_k,j_k)$.
\end{theorem}

%$Proof:$ 
\begin{proof}
We will prove this statement by induction on the power of the Kronecker product, k.

$Base \ Case:$ When k = 1, $K^k = K^1 = K$ is simply the initiator matrix. 
\\
\[v=
\begin{pmatrix}
	p_0&p_1&\ldots&p_{n^2-1}
\end{pmatrix} \rightarrow K = \begin{pmatrix}
	p_0&p_1&\ldots&p_{n-1}\\
    p_n&\ldots&\ldots &p_{2n-1}\\
    \vdots&\ddots&\ddots&\vdots\\
    p_{n^2-n}&\ldots&\ldots&p_{n^2-1}
\end{pmatrix}\]
Here the probability values are simply arranged in the matrix in numerical order, so $I$ uniquely decomposes to $(i,j)$ by $I = i*n+j$, where n is the size of the initiator matrix. This satisfies the Morton code because the interleaving of the values $i$ and $j$ produces the value $ij_n$ in base $n$, which also equals $in+j$.

$Inductive \ Step:$ Assume $M$ correctly maps between $K^k$ and $v^k$. Recall that $K^{k+1} = K^{k} \otimes K$. So each probability sequence in $K^{k+1}$, is simply the product of the probability sequences in the previous Kronecker matrix, $K^{k}$, and the initiator matrix probability values.

Let $p_1p_2 \ldots p_k p_{k+1}$ be a sequence in $v^{k+1}$. Then notice that $p_1p_2 \ldots p_k$ is a sequence in $v^k$. By assumption, the Morton code correctly gives the correct row and column values in $K^k$: $i_k$ and $j_k$. Then the row value for $p_1p_2 \ldots p_k p_{k+1}$ is $i_{k+1}$ where
\begin{align} 
i_{k+1} = i_k + \left\lfloor {\frac{val}{n}} \right\rfloor n^k
\label{eqn:rowval}
\end{align}
and $val$ is the index of $p_{k+1}$ in $v^{k+1}$. The reasoning for this is as follows. The size of the previous iteration's matrix, $n^k$, determines how large each ``row" is. When we multiply a probability sequence by a new value, think of ``zooming'' into a specific region of the Kronecker matrix. The region we ``zoom'' into is dependent on the position of the probability value. %The row location of a probability value can be found by simply taking the floor of the probability index divided by n.


The same reasoning can be translated to find the column index, $j_{k+1}$. 
\begin{align}
j_{k+1} = j_k + (val \% n) *n^k
\label{eqn:colval}
\end{align}
where $\%$ represents the modulus operator. By finding $val$ mod $n$, we know how many columns over the added probability value is. The morton code interleaves the digits of $i_{k+1}$ and $j_{k+1}$ in base $n$. $i_{k+1}$ in base $n$ is simply the digits of $i_k$ in base $n$ with the value $\lfloor {\frac{val}{n}} \rfloor$ added to the front. This is because the added value will occupy the $n^k$ digits place because that is what it is multiplied by in \ref{eqn:rowval}. Thus, the interleaved digits of $i_{k+1}$ and $j_{k+1}$ will be $\lfloor {\frac{val}{n}} \rfloor$, $(val \% n)$, followed by the interleaved digits of $i_k$ and $j_k$. Since, $I$ = interleaved digits of $i_k$ and $j_k$ in base $n$, it suffices to show that: 
\begin{align}
I_{k+1} = \lfloor {\frac{val}{n}} \rfloor *n^{2k+1} + (val \% n)*n^{2k} + I
\label{eqn:interleaved}
\end{align}
We multiply the first two digits by $n^{2k+1}$ and $n^{2k}$ respectively because those are the place values they occupy when moving from base $n$ to base $10$. Now we must find a way to express $I_{k+1}$ recursively in terms of $I_k$, $val$, and $n$. 

A given probability string s has a lexicographic index $I_k$. When we move to the next Kronecker power, we multiply this probability sequence by a third value, $val$. We can determine the new lexicographic index $I_{k+1}$ if we know $I$ and $val$. $I_{k+1} = I_k + val*(n^2)^k$ This result arises because we must add the number of permutations that start with values that precede $val$. The number of permutations that start with values before $val$ is simply the number of values that precede $val$, which span from $0$ to $val-1$, times the number of length $k$ permutations of initiator matrix probability values. There are $n^2$ probability values and $k$ slots to place them in with replacement so there are $v(n^2)^k$ permutations that start with values before $val$. We can now substitute this equation into equation \ref{eqn:interleaved} yielding $I_k + val*(n^2)^k = \lfloor {\frac{val}{n}} \rfloor *n^{2k+1} + (val \% n)*n^{2k} + I_k$. Simplifying yields $val = \lfloor {\frac{val}{n}} \rfloor *n + (val \% n)$. 

From here our proof is trivial because this equation is just a restatement of the remainder theorem. $val$ can be written as the integer portion of $val/n$ plus the remainder of $val$ divided by $n$. This completes our proof because we have shown that Morton code provides the correct map from $(i,j)$ indices of a probability sequence in the KPGM to the lexicographic index $I$ of the sequence.
\end{proof}

\subsection{Finding the Next Subregion}
After unranking the edges in an \ERfull subregion, the next step is to find the subsequent \ERfull subregion. For example, after finishing the ``$aabc$'' subregion of a $4^{th}$ power Kronecker graph, we must move on to the ``$aabd$'' subregion, because it is the next nondecreasing sequence of initiator matrix probability values. Once we have updated to the next subregion, we will repeat the process of hopping edges and unranking. 

This update algorithm works by first checking if the given array has a length of $1$. If so, the value is incremented by $1$. In the case that the value is the maximum, the value is changed to $-1$ to indicate that all \ERfull subregions have been completed. If the length of the array is greater than $1$, then the last element is incremented. In the case that the last element is the maximum, then the last element is changed to the final element of the updated version of a sub-array with the last element of the initial array removed. This step is taken to ensure that the returned sequence is non-decreasing so that no \ERfull subregion is generated twice. 

\subsection{Generating an Example Graph}
In this section, we generate a sample graph to illustrate the overall algorithm. Let's start with the 3 x 3 initiator matrix \\
\[P=
\begin{pmatrix}
	.4&.7&.55\\
    .3&.8&.9\\
    .5&.2&.6
\end{pmatrix}
\]
We would like to generate second power kronecker graph, which will have 9 nodes using this initiator matrix P, so we call $sample\_kronecker\_fast([[.4,.7,.5],[.3,.8,.9],[.5,.2,.6]],2)$. \\
\[P \otimes P = \begin{pmatrix}
	.16&.28&.22&.28&.49&.385&.22&.38&.3025\\
    .12&.32&.36&.21&.56&.63&.165&.44&.495\\
    .2&.08&.24&.35&.14&.42&.275&.11&.33\\
    .12&.21&.165&.32&.56&.44&.36&.63&.495\\
    .09&.24&.27&.24&.64&.72&.27&.72&.81\\
    .15&.1&.18&.4&.16&.48&.45&.18&.54\\
    .2&.35&.275&.08&.14&.11&.24&.42&.33\\
    .15&.4&.45&.06&.16&.18&.18&.48&.54\\
    .25&.1&.3&.1&.04&.12&.3&.12&.36\\
\end{pmatrix}\]

Here, each entry in $P \otimes P$ represents the probability that a cell in the random graph will contain an edge, or 1. As noted in section 1, the edges can be generated by either flipping a weighted coin at every single cell, or by hopping directly from edge to edge in each common probability region by drawing geometric random variables. An example of a randomly generated graph can be seen in figure \ref{example graph}.

\begin{figure}[ht]
\centering
\includegraphics[width=.45\textwidth]{6-12_sample_graph.png}
\caption{Sample Kronecker Graph with 9 nodes created using probability matrix found in section 4}
\label{example graph}
\end{figure}

\subsection{Efficiency Analysis}
Here we calculate the order of complexities of this algorithm and the previous coin flipping method. \newline
Coin Flipping – Recall that this method involves going through every pair of nodes (or cell of the adjacency matrix) and flipping a weighted coin. This algorithm takes $\bigO(k N^2) = \bigO(N^2 \log N)$ time, because finding the probability of a cell takes k, or $\log N$ time. (N is the number of nodes)
\newline
Grass Hopping – Recall that this method has the advantage of hopping directly to the next edge using the geometric random variable. The method takes approximately $\bigO(kE)$ time because we need only backward map the created edges. $E$ is the expected number of edges which can be calculated using indicator functions. For a given cell X, if $p(X=1)=s$, then the expected value of the cell is s. Because the total number of expected edges is just the sum of the indicator random variables of every cell, $E(E) = \sum_{i} p_i = 1$. 

In order to quickly sum up every single probability value, recall from Section 3.1 that every length k permutation with not necessarily distinct elements of a’s, b’s, c’s, and d’s appears in the matrix. By the multinomial theorem, the expansion of $(a+b+c+d)^k$ produces all of these such sequences. To prove that the time complexity is less than that of coin-flipping, multiply this expression by $N^2/N^2$. $N = 2^k$ so $N^2 = 4^k.$ Thus $E(E) = (a+b+c+d)^k \frac{N^2}{4^k} = N^2 (\frac{a+b+c+d}{4})^k$.
The average of a, b, c, and d is less than or equal to one, thus the expected number of edges is significantly less than $N^2$, especially for a large Kronecker power.  Let $\bar{p} = \frac{a+b+c+d}{4}$, then the order of complexity is $\bigO(N^2 \times \bar{p}^{\log n} \times \log n)$ which is significantly less than $\bigO(N^2 \times \log n)$.

\section{Fixed Edge Generation of Erd\H{o}s-R\'{e}nyi Graphs}
In the first section, we noted how the original \ERfull graph was one randomly sampled from the set of graphs with m edges and n nodes. We stumbled upon a potentially unknown method of generating such graphs using techniques detailed earlier in this paper. In a graph with n nodes, there are $\binom{n}{2}$ pairs of nodes or possible edges. Any subset of m pairs of nodes defines a unique graph. Thus there are $\binom{\binom{n}{2}}{m}$ possible graphs. How do randomly generate one of these graphs? Our solution is to ``rank" each graph by assigning it a numerical value from 0 to $\binom{\binom{n}{2}}{m}-1$. Once we randomly generate one of these ranks, we must unrank this value back to the m edges, and then unrank these edges back to pairs of nodes. Each graph is defined by set of edges, each of which can also be assigned a rank from 0 to $\binom{n}{2}-1$. We need a one-to-one correspondence between the graph rank and the set of edges that defines the graph. We can simply use a lexicographic map of non-decreasing sequences, similar to the solution to the unranking problem in section 3.2.1 i.e. if m=3, the following  ranks of graphs map to the following edges. $0->(0,1,2), 1->(0,1,3)$ and so on. We can generalize this mapping by writing an algorithm that takes 3 inputs: a rank, the maximum number of an edge, and the number of edges of our graph. The $unrank$ algorithm shown below will find the non-decreasing sequence in lexicographic order which satisfies the given parameters. Like the previous unranking algorithm, we must find the next element of our set by counting the number of possible sequences starting with that value. Instead of using the multinomial theorem though, we must use a combination because since the order of edges does not matter, each edge sequence has a unique non-decreasing ordering. 

The $erdos\_renyi$ algorithm uses the $unrank$ algorithm to generate a random graph from the set of $\binom{\binom{n}{2}}{m}-1$ graphs with n nodes and m edges. After randomly generating the "rank" of the graph, and finding the set of edges using the $unrank$ method, we must find the nodes that correspond to these edges. We can simply use the same $unrank$ algorithm to establish a one-to-one correspondence between the edge ranks and the ranks of the nodes. In this case, length = 2, because each edge has 2 nodes, and $max\_val$ = n because there are n nodes.

\begin{listing}
\caption{A simple code to generate an \ERfull graph with a fixed number of edges}
\label{code:fixed_er}
\begin{minted}{python}

# combination takes as input
#   n: the total number of objects to choose from
#   k:the number of objects to choose
# and returns the combination n choose k.
def combination(n,k): 
  return int( reduce(mul, (Fraction(n-i, i+1) for i in range(k)), 1) )

# unrank takes as input
#   I: the rank of the graph
#   max_val: the number of potential edges
#   length: the number of edges
# and returns the Ith non-decreasing sequence of edges
# of length 'length' and maximum edge of value of (max_val-1)
def unrank(I, max_val, length):
  array = [];
  # finds the next edge value
  for i in range(max_val):
    if length == 0:
      break;
    if length == 1:
      array.append(i + I);
      length=length-1;
    # checks if next edge value is i
    elif(combination(max_val-i-1, length-1) > I):
      array.append(i);
      length = length - 1; 
    else:
      I = I - combination(max_val-i-1, length-1);
  return array;

# erdos_renyi takes as input:
#   n: the number of nodes
#   m: the number of edges
# And generates a graph at random from the set of graphs
# with n nodes and m edges.

def erdos_renyi(n,m):
  graph = nx.Graph();
  #computes the number of possible edges
  possible_edges = int(n*(n-1)/2);
  #computes the number of possible graphs
  possible_graphs = int(combination(possible_edges,m));

  #randomly generates a "rank" or number of the graph
  I = int(random.random()*possible_graphs)

  #finds the m edges that make up the graph
  edges = unrank(I, possible_edges, m);

  #finds the nodes of edges: a set of edges.
  for edge in edges:
    nodes = unrank(edge, n, 2);
    print(nodes);
    graph.add_edge(nodes[0],nodes[1]);
  return graph;
\end{minted}  
\end{listing}


==> Stars_and_Bars.tex <==
%% Some definitions in order to build my figure

\def\starsandbars#1{{\ensuremath{%
  \edef\starlist{#1}%
  \foreach \i [count=\a] in \starlist{%
    \ifnum\a>1\big|\fi%
    \ifnum\i>0\foreach \j in {1,...,\i}{\star}\fi%
  }}}}%
  

%% Figure below
\begin{figure}[h]
\centering
$\foreach \j in {1,...,15}{\star}$ \\
$\Downarrow$ \\
\foreach \i in {{4,3,2,6}, {1,7,3,4}}{\leavevmode 
\starsandbars{\i} \par
}
\caption{A simple stars and bars example. $k = 15$ stars are split among 3 dividers.}
\label{fig:stars_and_bars}
\end{figure}
